Personalized Federated Deep Reinforcement Learning for Heterogeneous Edge Content Caching Networks

Proactive caching is essential for minimizing latency and improving Quality of Experience (QoE) in multi-server edge networks. Federated Deep Reinforcement Learning (FDRL) is a promising approach for developing cache policies tailored to dynamic content requests. However, FDRL faces challenges such as an expanding caching action space due to increased content numbers and difficulty in adapting global information to heterogeneous edge environments. In this paper, we propose a Personalized Federated Deep Reinforcement Learning framework for Caching, called PF-DRL-Ca, with the aim to maximize system utility while satisfying caching capability constraints. To manage the expanding action space, we employ a new DRL algorithm, Multi-head Deep Q-Network (MH-DQN), which reshapes the action output layers of DQN into a multi-head structure where each head generates a sub-dimensional action. We next integrate the proposed MH-DQN into a personalized federated training framework, employing a layer-wise approach for training to derive a personalized model that can adapt to heterogeneous environments while exploiting the global information to accelerate learning convergence. Our extensive experimental results demonstrate the superiority of MH-DQN over traditional DRL algorithms on a single server, as well as the advantages of the personal federated training architecture compared to other frameworks.

==> performance.tex <==
\section{Performance Evaluation}
%In this section, we use simulations to numerically evaluate the performance of the proposed algorithms.

\subsection{Experimental Settings}
We consider there are five MEC servers within the system, and the system includes two types of heterogeneity: content popularity and user distribution.
We model heterogeneous content popularity by setting different MZipf plateau factors and Zipf factors in Eq.~\eqref{mzipf}~\cite{WangC}, 
and assume the number of users within the coverage area of each MEC server is not the same to simulate the heterogeneous user distribution. For the user distribution, we assume that the number of users within the coverage area of each MEC server is not the same.
The DNN structures of proposed algorithms are implemented by the deep learning library PyTorch~1.8. 
%We use the following parameters:
%the learning rate $\xi = 0.002$, 
%the size of mini-batch is $128$,
%the reward discounted factor $\gamma = 0.99$ and 
%the update coefficient $\tau = 0.005$.
The detailed default experimental parameters are listed in Table~\ref{para}.
%Experiments are conducted on 32 CPU cores of an AMD Epyc server with 2TB of RAM. An NVIDIA A100 GPU is used for DNN computations.
%\vspace{-2ex}
\iffalse
\begin{table}[!t]
	\begin{center}
		\caption{Simulation Parameters}
		\label{para}
		\begin{tabular}{|c|c|} \hline
			\textbf{Parameter} &  \textbf{Value} \\\hline
			Number of MEC servers $M$ & $5$  \\ \hline
			Plateau factors of MZipf $q_m$ & $[100, 200, 90, 40, 80]$\\ \hline
			Zipf factors of MZipf $k_m$ & $[0.60, 0.60, 0.75, 0.90, 0.90]$\\ \hline
			%					Number of time slots $T$ & $200$ \\ \hline
			Data size of contents $\eta_c$ & $1\sim8$ GB \\ \hline
			Downloading payment of contents $\phi_c$ & $0.05\sim0.5$ HKD \\ \hline
			
			Number of DNN layers & $6$ \\ \hline
			Number of neurons per hidden layer & $128$ \\ \hline
			%					 Size of mini-batch & $128$ \\ \hline
			Learning rate $\xi$ & $0.002$ \\ \hline
			Update coefficient $\tau$ & $0.005$ \\ \hline
			Discounted factor $\gamma$ & $0.99$ \\ \hline
		\end{tabular}
	\end{center}
 \vspace{-0.2in}
\end{table}
\fi

\begin{table}[!t]
	\begin{center}
		\caption{Simulation Parameters}
		\label{para}
		\begin{tabular}{cc} % 去掉了竖线
			\toprule % 使用 top rule
			\textbf{Parameter} & \textbf{Value} \\
			\midrule % 使用 mid rule
			Number of MEC servers $M$ & 5 \\
			Plateau factors of MZipf $q_m$ & [100, 200, 90, 40, 80] \\
			Zipf factors of MZipf $k_m$ & [0.60, 0.60, 0.75, 0.90, 0.90] \\
			Data size of contents $\eta_c$ & 1$\sim$8 GB \\
			Downloading payment of contents $\phi_c$ & 0.05$\sim$0.5 HKD \\
			Number of DNN layers & 6 \\
			Number of neurons per hidden layer & 128 \\
			Learning rate $\xi$ & 0.002 \\
			Update coefficient $\tau$ & 0.005 \\
			Discounted factor $\gamma$ & 0.99 \\
			\bottomrule % 使用 bottom rule
		\end{tabular}
	\end{center}
\end{table}
\subsection{Performance Evaluation of MH-DQN Algorithm}
In this subsection, we set the number of contents to $40$ and evaluate the effectiveness of the MH-DQN algorithm for a single MEC server. 
%Specifically, We set the number of contents to $40$ and elaborate the performance of multi-head output layers framework on a single server.
%on a single edge server in terms of convergence speed and system utility
Since traditional DQN cannot handle such a large action space, we use continuous algorithm PPO~\cite{WangY} with a sampling process in the same environment for comparison. 

The results across multiple metrics consistently show the superiority of our proposed MH-DQN approach over the baseline PPO. In Fig.~\ref{ppo}(a), which displays MEC utility, MH-DQN demonstrates a significant improvement, stabilizing at approximately 0.35 after an initial rise. In contrast, PPO shows greater fluctuation and achieves lower utility values consistently. Fig.~\ref{ppo}(b) shows the CHR, where MH-DQN reaches a stable peak close to 0.40, whereas PPO exhibits lower and more variable CHR values. Fig.~\ref{ppo}(c) illustrates replacement costs, where MH-DQN's costs decrease quickly and remain low, indicating efficient resource management. On the other hand, PPO's costs are higher and display more fluctuations. In  Fig.~\ref{ppo}(d), concerning penalties, MH-DQN quickly reduces penalties to nearly zero, showing its effectiveness in minimizing operational drawbacks. PPO, however, maintains higher levels of penalties throughout the episodes.

We also observe that PPO exhibits higher policy entropy fluctuations, suggesting issues with premature convergence or unstable learning dynamics arising from directly optimizing the high-dimensional caching policy over the exponentially large action space. Our MH-DQN framework solves this through the factorized multi-head representation, which reduces policy sensitivity to parameter updates, enabling smoother convergence. Additionally, the target network architecture provides consistent value estimates, further stabilizing the training process and mitigating oscillations. Consequently, MH-DQN learns more coherent and stable caching policies, as evident from the steadily decreasing entropy trajectory, contributing to its superior overall performance in terms of utility, cache hit ratio, replacement cost, and learning stability.




%The results in Fig.~\ref{ppo} show that the CHR of both algorithms increases with the increase of training episodes,  while the replacement cost and penalty are decreasing,  so the utility of the MEC server is increasing. However, there is still a significant difference in terms of convergence speed and final utility between these two algorithms. With multi-head architecture, MH-DQN converges faster and outperforms PPO. Our proposed framework enables the Q-network to output discrete actions directly without the additional transformation.  Additionally, as each head in MH-DQN is computed in parallel, the training parameters are reduced, speeding up the convergence process.
%\vspace{-2ex}
\begin{figure}[!t]
	\centering
	\includegraphics[width=0.95\linewidth]{pics/vs.pdf}
	\caption{Performance comparison of modified DQN and PPO algorithm.}
	\label{ppo}
 \vspace{-0.1in}
\end{figure}
\vspace{-1ex}
\subsection{Performance Evaluation of PF-DRL-Ca Algorithm}
We evaluate and compare the performance of the PF-DRL-Ca algorithm with two learning-based algorithms and three non-learning caching approaches, which are presented as follows.
\romannumeral1) \textit{NonPer}: A conventional FDRL framework without the personalized layers. It can also be viewed as the number of personalized layers is $0$;
\romannumeral2) \textit{NonFed}: A conventional DRL framework without the FL paradigm. It can also be viewed as the number of personalized layers equals $6$;
\romannumeral3) \textit{LRU}~\cite{HuangQ}: A non-learning approach in which the least recently used contents will be replaced;
\romannumeral4) \textit{LFU}~\cite{HuangQ}: A non-learning approach in which the least frequently used contents will be replaced;
\romannumeral5) \textit{Random}: A non-learning approach in which content caching decisions are generated randomly.
%
%
%\begin{itemize}
%	\item \textit{NonPer}: A conventional FDRL framework without the personalized layers. It can also be viewed as the number of personalized layers is $0$;
%	
%	\item \textit{NonFed}: A conventional DRL framework without the FL paradigm. It can also be viewed as the number of personalized layers equals $6$;
%	
%	\item \textit{LRU}~\cite{HuangQ}: A non-learning approach in which the least recently used contents will be replaced;
%	
%	\item \textit{LFU}~\cite{HuangQ}: A non-learning approach in which the least frequently used contents will be replaced;
%	
%	\item \textit{Random}: A non-learning approach in which content caching decisions are generated randomly.
%\end{itemize}


%We first compare the convergence performance of three learning-based algorithms, and the result is shown in Fig.~\ref{converagence}. In Fig.~\ref{converagence}, each curve is accompanied by a shaded region of similar color, representing the range of system utility of the MEC servers. The utility of all algorithms increases with the increase of training episodes and gradually reaches a plateau with small fluctuations. PF-DRL-Ca has the best final performance, NonPer comes second, and NonFed is the worst. Moreover, due to the lack of federated learning, the system utility gap between MEC servers in NonFed is the largest; while in NonPer, there is almost no performance gap between MEC servers; only PF-DRL-Ca achieves the optimal overall performance with an acceptable system utility gap.

\subsubsection{Convergence Performance} As shown in Fig.~\ref{converagence}, our proposed PF-DRL-Ca method outperforms the two baselines, NonPer and NonFed, in terms of both final converged utility and convergence speed. PF-DRL-Ca achieves the highest system utility while maintaining a relatively narrow shaded region, suggesting that it effectively balances overall performance and local personalization across MEC servers. In contrast, the NonFed approach, which lacks any federated collaboration, exhibits the lowest utility and the widest shaded region, indicating significant performance disparities among MEC servers. This is expected as the absence of knowledge sharing leads to incomplete training for each individual node, resulting in suboptimal and highly heterogeneous caching strategies. The NonPer method, while incorporating federated aggregation through the CCS, still underperforms PF-DRL-Ca. Despite achieving a narrower shaded region compared to NonFed, the lack of personalization in NonPer leads to a \textit{one-size-fits-all} global policy that fails to adapt to local user preferences, resulting in a lower overall utility.  By separating the neural network into shared base layers and personalized head layers, PF-DRL-Ca effectively captures both global patterns and local heterogeneities. The weighted aggregation of base layers prioritizes contributions from MEC servers with more user requests, further enhancing the global representation. Simultaneously, the personalized head layers enable each node to specialize in catering to its unique user population, leading to optimized caching strategies that strike the right balance between global coordination and local adaptation.


\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.7\linewidth]{pics/convergence.pdf}
	\caption{Convergence comparison of three DRL-based algorithms.}
	\label{converagence}
\end{figure}

\subsubsection{Effect of the number of personal layers}
%Fig.~\ref{NumOfPer} shows the system utility of the PF-DRL-Ca algorithm with different numbers of personalized layers. The PF-DRL-Ca algorithm can achieve the best performance by setting $4$ base layers and $2$ personalized layers. Fig.~\ref{NumOfPer} also shows that employing two personalized layers brings about $30\%$ and $330\%$ performance improvements compared to the NonPer and NonFed algorithms, respectively. So, it confirms that neither the base layers nor the personalized layers are redundant. Without the base layers, there are insufficient training samples to learn individual DQN models effectively.  Meanwhile, without the personalized layers, the servers are unable to handle the heterogeneity in their environments.

Fig.~\ref{NumOfPer} shows the impact of varying personalized layer counts on the system utility achieved by our PF-DRL-Ca algorithm. The utility initially increases as personalized layers are added from zero (NonPer baseline) up to an optimal point of two personalized layers, after which adding more layers provides no further benefit. Employing two personalized layers yields a significant 30\% utility gain over NonPer and a remarkable 330\% improvement compared to NonFed. This result highlights the importance of balancing shared global representations with localized personalization. Without shared base layers (zero personalized), there are insufficient samples to learn an effective generalized model. Conversely, with all layers personalized (six personalized), the algorithm fails to capture commonalities across servers, hindering knowledge sharing. The optimal configuration of four base layers and two personalized layers allows base layers to extract generalizable features from aggregated data, while personalized layers adapt to each server's unique user preferences. This synergy between global coordination and local specialization enables PF-DRL-Ca to learn highly effective, tailored caching strategies leveraging collective federated knowledge.

\begin{figure}[!b]
	\centering
	\includegraphics[width=0.7\linewidth]{pics/num of per.pdf}
	\caption{Performance comparison with different numbers of personalized layers.}
	\label{NumOfPer}
\end{figure}
%\vspace{-2ex}



\subsubsection{Effect of the number of contents}
%Fig.~\ref{ContentsNum} shows a performance comparison of all caching algorithms with different numbers of contents. We set the number of contents range from $40$ to $60$, The system utility of all algorithms decreases as the number of contents increases, which is caused by the increase in decision space.  From Fig.~\ref{ContentsNum}(a), the PF-DRL-Ca algorithm achieves the highest average CHR compared with all baselines. Moreover, the CHR gap between the proposed algorithm and the best other baseline becomes larger as the number of contents increases. Specifically, when the number of content is $60$, the CHR of the proposed algorithm is approximately $27\%$, $113\%$ and $56\%$ higher than that obtained by the NonPer, NonFed and non-learning schemes, respectively.  From Fig.~\ref{ContentsNum}(b), all the learning-based methods perform almost equally well in terms of average replacement cost, which is much lower than the non-learning methods. This is because the the DRL model enable servers to learn user request patterns, leading to better caching decisions at the beginning to avoid the replacement cost of frequent updates



Fig.~\ref{ContentsNum} presents a performance comparison of six caching algorithms as the number of contents varies. Fig.~\ref{ContentsNum}(a) depicts the average CHR for different algorithms as the number of contents increases from 40 to 60. We observe a declining trend in the CHR for all algorithms as more contents are introduced. This behavior can be attributed to the fixed cache capacity limitation. With a larger content catalog, the same cache size can hold a smaller fraction of the total contents, leading to a lower probability of requested contents being available in the cache, thereby reducing the overall CHR. Despite this general decline, our proposed PF-DRL-Ca algorithm consistently outperforms all baselines, maintaining the highest average CHR across the entire range of content numbers. Moreover, the performance gap between PF-DRL-Ca and the best alternative baseline widens as the number of contents grows, highlighting its effectiveness in optimizing cache utilization under increasing decision space complexity. Fig.~\ref{ContentsNum}(b) reveals that all learning-based methods, including PF-DRL-Ca, NonPer, and NonFed, exhibit comparable and significantly lower average replacement costs compared to the non-learning approaches, such as LRU and Random. This advantage can be attributed to the ability of DRL models to learn and adapt to user request patterns, enabling more informed caching decisions from the outset and minimizing the need for frequent cache replacements.


\begin{figure}[!t]
	\centering
	\includegraphics[width=\linewidth]{pics/contents num.pdf}
	\caption{Performance comparison with different numbers of contents in terms of: (a) CHR; (b) replacement cost.}
	\label{ContentsNum}
 \vspace{-0.1in}
\end{figure}
%\vspace{-1ex}

\subsubsection{Effect of the cache size and user dynamics}

Fig.~\ref{StorageSize} presents a performance comparison of different caching algorithms under varying storage sizes for each MEC server, ranging from 45 GB to 65 GB. As expected, the system utility of all algorithms increases with larger storage sizes. This trend is intuitive because a larger cache capacity allows more contents to be stored, increasing the likelihood of serving user requests from the cache and improving overall utility. Our proposed PF-DRL-Ca algorithm consistently outperforms all baselines across the entire range of storage sizes, achieving the highest system utility. Notably, the performance gap between PF-DRL-Ca and the other algorithms widens as the storage size increases, highlighting its ability to leverage the additional cache capacity through intelligent caching decisions.

Fig.~\ref{UsersNum} examines the performance of the same algorithms under different average numbers of users per MEC server. In this scenario, we observe an interesting trend: the system utility of PF-DRL-Ca and the NonPer baseline increases as the average number of users grows, while the utility of the NonFed and non-learning algorithms, like LRU and Random, decreases. This contrasting behavior can be attributed to the ability of learning-based algorithms, particularly PF-DRL-Ca, to adapt and optimize caching strategies based on user request patterns. With a larger user base, these algorithms can leverage more diverse request data to improve their caching policies, leading to better cache utilization and higher system utility. In contrast, the non-learning algorithms, such as LRU and Random, cannot adapt to changing user dynamics, resulting in suboptimal caching decisions and a decline in performance as the user base grows more diverse and complex. These experimental results demonstrate the robustness and effectiveness of our proposed PF-DRL-Ca algorithm in handling varying cache sizes and user dynamics, reinforcing its suitability for intelligent caching in dynamic edge computing environments.




\begin{figure}[!t]
	\begin{minipage}[t]{0.495\linewidth}
		\centering
		\includegraphics[width=\linewidth]{pics/storage size.pdf}
		\caption{Performance comparison with different storage sizes.}
		\label{StorageSize}
	\end{minipage}
	\begin{minipage}[t]{0.495\linewidth}
		\centering
		\includegraphics[width=\linewidth]{pics/users num.pdf}
		\caption{Performance comparison with different average numbers of users.}
		\label{UsersNum}
	\end{minipage}
 %\vspace{-0.2in}
\end{figure}
%\vspace{-1ex}







